Inferring Latent Domains for Unsupervised Deep Domain Adaptation

Unsupervised Domain Adaptation (UDA) refers to the problem of learning a model in a target domain where labeled data are not available by leveraging information from annotated data in a source domain. Most deep UDA approaches operate in a single-source, single-target scenario, i.e. they assume that the source and the target samples arise from a single distribution. However, in practice most datasets can be regarded as mixtures of multiple domains. In these cases, exploiting traditional single-source, single-target methods for learning classification models may lead to poor results. Furthermore, it is often difficult to provide the domain labels for all data points, i.e. latent domains should be automatically discovered. This paper introduces a novel deep architecture which addresses the problem of UDA by automatically discovering latent domains in visual datasets and exploiting this information to learn robust target classifiers. Specifically, our architecture is based on two main components, i.e. a side branch that automatically computes the assignment of each sample to its latent domain and novel layers that exploit domain membership information to appropriately align the distribution of the CNN internal feature representations to a reference distribution. We evaluate our approach on publicly available benchmarks, showing that it outperforms state-of-the-art domain adaptation methods.

==> img/confusion-pacs.tex <==
To further demonstrate the advantages of adopting a multi-source domain adaptation approach and the benefit of considering different statistics for aligning features of different domains, we conduct an additional analysis. Specifically, we consider the Multi-source DA method and analyze how the performance of the target classifier varies when adopting the batch normalization statistics of different domains.
%In this section we analyze the \massi{link} between the statistics of different domains within the PACS dataset.
%To this extent we take the multisource-DA model, which computes the exact statistics for each source domain.% perfect knowledge about the domain label of each sample. 
%Then we compute the results of classifying images of a the target domain using the statistics of one of the source domains. %when their features are aligned to the model through statistics computed for another domain. 
In other words, we substitute the statistics of DA layers for the target model with those associated to one of the source domains, observing how this change influences the performances. Of course, we also consider the case where the "right" statistics, \ie those corresponding to target domain, are used. %changing the statistics used for aligning the images can impact the classification performances of the model. 
We repeat this analysis for each possible combination of sources\slash{}target domains. 
%We can further analyze this aspect by considering the correlation between the statistics of the different source domains. %To this extent, for each setting of Table~\ref{tab:pacs}, we report the performances of the Multi-source DA model when the images of a domain are aligned using statistics of different domains. 
Figure \ref{fig:confusion-matrices} shows the results. Each group of four color bars indicates a different experiment (\ie a different target domain). 
 
\begin{figure}[t]
   \centering
  {\includegraphics[width=1\columnwidth]{img/cm-graph-sup.pdf}\label{fig:cm-photo}} 
    \caption{PACS dataset: classification accuracies of the Multi-source DA model as CNN feature representations of a domain are aligned using statistics of a different domain. % (color bars). %The Sketch domain has features which are distant from the other domains, especially natural images on which the network has been pretrained. At the same time, using the statistics of the Cartoon domain for classifying Sketch images does not produce a considerable drop in performances: without considering multiple source domains, it would be hard to take into account this similarity and effectively address this DA problem.
   }
   \label{fig:confusion-matrices}
 \end{figure}
 
As expected, when the statistics of Sketch are used, there is a huge drop in performances in every scenario (\ie when Photo, Art and Cartoon are considered as target) due to the distance of the feature distributions of this domain from those of the other domains. When Sketch is considered as target, %there is a significant drop in performances 
the accuracy decreases significantly
if the statistics of Photo or Art domains are employed. Instead, using the statistics derived from the Cartoon domain, higher accuracy is obtained. This is not surprising due to the similarity in visual appearance between images of the Cartoon and the Sketch domains.
Importantly, only a multi-source DA model can exploit this similarity, while traditional single-source approaches will not suffice. %model has no possibility of extracting the similarity between one of the source domains and the target. 
